Nearly Minimax Algorithms for Linear Bandits with Shared Representation

We give novel algorithms for multi-task and lifelong linear bandits with shared representation. Specifically, we consider the setting where we play $M$ linear bandits with dimension $d$, each for $T$ rounds, and these $M$ bandit tasks share a common $k(\ll d)$ dimensional linear representation. For both the multi-task setting where we play the tasks concurrently, and the lifelong setting where we play tasks sequentially, we come up with novel algorithms that achieve $\widetilde{O}\left(d\sqrt{kMT} + kM\sqrt{T}\right)$ regret bounds, which matches the known minimax regret lower bound up to logarithmic factors and closes the gap in existing results [Yang et al., 2021]. Our main technique include a more efficient estimator for the low-rank linear feature extractor and an accompanied novel analysis for this estimator.

==> header.tex <==

\usepackage{hyperref}

%\usepackage[authoryear,numbers,semicolon,square]{natbib}

%\usepackage{mathpazo}
%\usepackage{euler}

\usepackage{url}
\usepackage{amsthm, amssymb}
\usepackage{verbatim}
\usepackage[inline]{enumitem}
\usepackage{xcolor}
\usepackage{pgf}

\hypersetup{
  colorlinks   = true, %Colours links instead of ugly boxes
  urlcolor     = blue, %Colour for external hyperlinks
  linkcolor    = blue, %Colour of internal links
  citecolor   = blue %Colour of citations
}
\setlist[enumerate, 1]{label=(\alph*)}
\setlist[enumerate]{nosep}

\theoremstyle{plain}
\newtheorem{thm}{Theorem}
%\newtheorem{prop}[thm]{Proposition}
\newtheorem{lem}{Lemma}
\newtheorem{coro}[thm]{Corollary}
\newtheorem{fact}[thm]{Fact}

\theoremstyle{definition}
\newtheorem{defn}{Definition}
\newtheorem{assum}{Assumption}
%\newtheorem{ex}{Exercise}
%\newtheorem{eg}{Example}
%\newtheorem{prob}{Problem}

\theoremstyle{remark}
\newtheorem{claim}{Claim}
\newtheorem{rem}{Remark}


%\renewcommand{\algorithmautorefname}{Algorithm}
\newcommand{\lemautorefname}{Lemma}
\newcommand{\defnautorefname}{Definition}
\newcommand{\propautorefname}{Proposition}
\newcommand{\thmautorefname}{Theorem}
\newcommand{\factautorefname}{Fact}
\newcommand{\assumautorefname}{Assumption}
\newcommand{\coroautorefname}{Corollary}
\renewcommand{\sectionautorefname}{Section}
\renewcommand{\subsectionautorefname}{Section}
%\renewcommand{\algorithmcflinename}{Line}


\renewcommand{\eqref}[1]{\hyperref[#1]{(\ref{#1})}}


\newcommand{\algoname}{$\mathsf{E^2TC}$}



\newcommand{\red}[1]{#1}%\textcolor{red}{#1}}
